Identifying frequency decorrelated dust residuals in B-mode maps by exploiting the spectral capability of bolometric interferometry

Astrophysical polarized foregrounds represent the most critical challenge in Cosmic Microwave Background (CMB) B-mode experiments. Multi-frequency observations can be used to constrain astrophysical foregrounds to isolate the CMB contribution. However, recent observations indicate that foreground emission may be more complex than anticipated. We investigate how the increased spectral resolution provided by band splitting in Bolometric Interferometry (BI) through a technique called spectral imaging can help control the foreground contamination in the case of unaccounted Galactic dust frequency decorrelation along the line-of-sight. We focus on the next generation ground-based CMB experiment CMB-S4, and compare its anticipated sensitivities, frequency and sky coverage with a hypothetical version of the same experiment based on BI. We perform a Monte-Carlo analysis based on parametric component separation methods (FGBuster and Commander) and compute the likelihood on the recovered tensor-to-scalar ratio. The main result of this analysis is that spectral imaging allows us to detect systematic uncertainties on r from frequency decorrelation when this effect is not accounted for in component separation. Conversely, an imager would detect a biased value of r and would be unable to spot the presence of a systematic effect. We find a similar result in the reconstruction of the dust spectral index, where we show that with BI we can measure more precisely the dust spectral index also when frequency decorrelation is present. The in-band frequency resolution provided by BI allows us to identify dust LOS frequency decorrelation residuals where an imager of similar performance would fail. This opens the prospect to exploit this potential in the context of future CMB polarization experiments that will be challenged by complex foregrounds in their quest for B-modes detection.

==> II/II-2/The_QUBIC_Instrument.tex <==
\st{QUBIC is the first CMB B-mode experiment based on bolometric interferometry. The instrument observes the sky in two frequency bands, centered at 150~GHz and 220~GHz, respectively, with a 25$\%$ bandwidth.} \st{Each feed-horn array is made of 400+400 back-to-back antennas and each focal plane is equipped with 992 TES bolometers.} \st{QUBIC will observe from the Alto Chorrillos site, in the Argentinian Andes, at about 5000 meters a.s.l. and will provide an upper limit on $r<0.015$ at $68\%$ C.L. after three years of observations}% \citep{2020.QUBIC.PAPER1}.

\st{The first QUBIC prototype is referred to as the  \textit{technological demonstrator} (TD), a reduced version of the instrument to demonstrate bolometric interferometry with laboratory measurements and sky observations. The QUBIC-TD uses the same cryostat} \citep{Masi_2022}, HWP \citep{D_Alessandro_2022} \st{and polarizing grid as the final instrument, but will observe only in the 150 GHz channel. It is equipped with smaller diameter mirrors, a smaller feed-horn array made of 64+64 back-to-back feed-horns, and a smaller focal plane, made of 248 bolometers.}

\st{After extensive laboratory testing the QUBIC-TD was installed at the observation site during November 2022} (see Fig.~\ref{fig:QUBIC_Rendering}). \st{Routine observations will start after commissioning.} \st{The interested reader can find the details of the laboratory tests and their results in:}% \citet{2020.QUBIC.PAPER1, 2020.QUBIC.PAPER2, 2020.QUBIC.PAPER3, 2020.QUBIC.PAPER4, 2020.QUBIC.PAPER5, 2020.QUBIC.PAPER6, 2020.QUBIC.PAPER7, 2020.QUBIC.PAPER8}.

\st{The top-left panel of figure}~\ref{fig:SB_meas_vs_theo} \citep[taken from][]{2020.QUBIC.PAPER1} \st{shows the synthesized beam measured by one of the focal plane TES detectors compared to a simulation of the same beam (top-right panel). The bottom panel of the same figure} \citep[taken from][]{2020.QUBIC.PAPER3} \st{shows the synthesized beams measured at various frequencies. These data show the multiple-peaked shape of the synthesized beam with good agreement with the theoretical predictions and the expected frequency dependence of the secondary peak positions. The measured instrumental noise (detectors and read-out) is $2.06\times 10^{-16}\,\mathrm{W}/\sqrt{\mathrm{Hz}}$} \citep{2020.QUBIC.PAPER4} \st{and the median cross-polarization of the detectors is $0.12\%$ }\citep{2020.QUBIC.PAPER6}.


%\begin{figure}[ht]
%	\includegraphics[width=9cm]{II/II-2/Qubic_on_site.png} %II/II-2/
%        \caption{QUBIC-TD in the Alto Chorrillos site. The cryostat is placed on a movable mount to scan in azimuth and elevation. The system is placed inside a motor-controlled dome that can be opened and closed.}
%     \label{fig:QUBIC_Rendering}
%\end{figure}
% 
\begin{figure}[ht]
	\includegraphics[width=9cm]{II/II-2/SB_data_vs_theory_new.png}\\
	\mbox{}\\
	\includegraphics[width=9cm]{figure/SB_vs_frequency_mod.pdf}
        \caption{\label{fig:SB_meas_vs_theo}\textit{Top panel}: synthesized beam measured for one detector at 150\,GHz (left) compared with the  simulated 150\,GHz synthesized beam for the same detector \citep[right, from][]{2020.QUBIC.PAPER1}. \textit{Bottom panel}: synthesized beam for one detector measured at various frequencies \citep[from][]{2020.QUBIC.PAPER3}.}
     
\end{figure}


==> III/III-1/III-1-3/fgbuster_vs_commander.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                  %%
%%  This is a LaTeX2e table fragment exported from Gnumeric.        %%
%%                                                                  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[h!]
    \caption{\label{tab:fgbuster_vs_commander}Parameters used in the simulations with FGBuster and Commander. \red{Togliere colonna Commander, cambiare sky patch FGBuster (0 -45)}}
    \renewcommand{\arraystretch}{2}
    \begin{center}
        \begin{tabular}{p{2.5cm} m{2cm} m{2cm}}
            \hline
            & \makecell[c]{FGBuster} & \makecell[c]{Commander} \\ 
            \hline
            \hline
            \makecell[l]{N. realizations\\ \mbox{}[CMB and noise]\dotfill}	& \makecell[c]{500} & \makecell[c]{100$^1$}\\
            Map $N_\mathrm{side}$\dotfill	& \makecell[c]{256} & \makecell[c]{\phantom{0}64$^1$}\\
            Multipole range\dotfill	&\centering 21--335 &\makecell[c]{21--128$^2$}\\
            $\Delta\ell$\dotfill &\multicolumn{2}{c}{\phantom{0}{35}} \\
            Input $r$\dotfill & \multicolumn{2}{c}{\phantom{00}{0}} \\
            \makecell[l]{Residual lensing\\ fraction\dotfill} & \makecell[c]{\\ \phantom{000}10\%$^3$} & \makecell[c]{\\ \phantom{00}100\%$^3$}\\
            Sky fraction [\%]\dotfill & \multicolumn{2}{c}{\phantom{0000}3\%} \\
            \makecell[l]{Sky patch center\\ \mbox{}[Equatorial coord.]\dotfill} & 
                \makecell[c]{$\alpha=-30^\circ$\\\phantom{1}$\beta=-30^\circ$$^4$}&\makecell[c]{$\alpha=\phantom{-0}0^\circ$\\\phantom{1}$\beta=-57^\circ$$^5$}\\
            \makecell[l]{Smoothing with\\Gaussian beam\dotfill} & \centering None&\makecell[c]{\phantom{00}1$^\circ$}\\
            \hline
            \multicolumn{3}{l}{\makecell[l]{
            \footnotesize{$^1$Limited by computational time.}\\
            \footnotesize{$^2$Limited by $N_\mathrm{side}=64$} \\
            \footnotesize{$^3$This is the fraction of the lensing signal left in the CMB map.}\\
            \footnotesize{\phantom{$^3$}The value of 100\% means that all the lensing signal was left }\\
            \footnotesize{\phantom{$^3$}in the map, in the other case only the 10\% of the lensing remains.}\\
            \footnotesize{$^4$Center of sky patch represented by the light region in Fig.~\ref{fig:sky_patches}.} \\
            \footnotesize{$^5$Center of sky patch observed by QUBIC (dark region in Fig.~\ref{fig:sky_patches}).} 
            }}
        \end{tabular}
    \end{center}
\end{table}

% \begin{tabular}{|m{3cm}|m{5cm}|}
% \hline
% \makecell[c]{Column 1} & \makecell[c]{Long text that \\ needs to be wrapped} \\ [0.5ex] 
% \hline
% \makecell[c]{Cell 1} & \makecell[c]{Long text that \\ \textbackslash{}[needs to be wrapped} \\ [1ex] 
% \hline
% \end{tabular}


==> III/III-2/III-2-1/simple.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{figure/figlike.png}
    \caption{{\bf a)} Histograms of the reconstructed $r$ in the case of r=0 and the {\bf d1s1} model (smoothed using Kernel Density Estimator) for a number of sub-dbands ranging from 1 (classical imager - CMB-S4 current design) to 8 using bolometric interferometry.  {\bf b)} Same but with r=0.01 and the {\bf d1s1} model. {\bf c)} Same but with r=0 and the {\bf d6s1} model where Dust decorrelation (with $\ell_{corr}=10$) induces a significant bias that reduces with the number of sub-bands.
    {\bf d)} Evolution of the mean and standard-deviation of the histograms for {\bf d1s1} and {\bf d6s1}.}
    \label{fig:like_d1}
\end{figure*}

 The first model we explore here is the simplest one where spectral indices for thermal dust and synchrotron radiation are constant across the sky. This corresponds to {\bf d0s0}, model 1 of the section~\ref{sec_simulated_sky_model}. The simplicity of this model result makes it computationally efficient. \\

\begin{table}[H]
	\centering
	\caption{Recovered parameters for {\bf d0s0}:}
	\label{tab:params_simple}
	\begin{tabular}{lccr} % 2 columns, alignment for each
		\hline
		$r$ bias & $3.0 \times 10^{-5}$ \\ 
		$\sigma(r)$ & $4.998 \times 10^{-4}$ \\ 
		Dust spectral index $\beta_d$ & $1.540 \pm 2.13 \times 10^{-3}$ \\
		Synchrotron spectral index $\beta_s$ & $-3.000 \pm 7.43 \times 10^{-4}$ \\
		\hline
	\end{tabular}
\end{table}

We performed simulations with 500 realizations of CMB and noise. Table~\ref{tab:params_simple} summarizes the main results of the pipeline in this simple case with constant spectral indices across the sky. We obtain an unbiased estimate of the spectral indices, resulting in low foreground residuals in our maps.
As a result, we find a very small bias on $r$ with a standard deviation very close to that found in \cite{Abazajian_2022} with the same configuration. 



==> III/III-2/III-2-2/varying_index.tex <==

In the previous section, considered the case of a simple model with constant indices across the sky. This is clearly an oversimplified case~\citep{Planck_15}. Let's now consider a model with foreground spectral indices that varies across the sky. Our simulated foregrounds have inputs $\beta$ maps with a pixelization $N_{\text{side}} = 256$, based on the results from  \cite{Planck_15}. For computational reasons and in order to be more realistic, the fit of our spectral indices during component separation is performed with a coarser pixelization $N_{\text{fit}} = 8$. We expect this to introduce a slight bias on the spectral indices recovered during component separation, resulting in foreground residuals in our maps and therefore induce a small bias on $r$. 
%\\ {\color{red}[I suggest to expand on this a bit: this gives a bias if we look at the product of the likelihoods, but on the average likelihood we don't see a bias (see fig \ref{fig:result_r_vs_dust_model}: the model d1 is is consistent with the input r)]}.

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.45]{figure/d1_recon_r.png}
%     \caption{{\color{red}Clear this fig}Likelihood for the case of a classical imager ($N_{\text{sub}} = 1$) and a bolometric interferometer ($N_{\text{sub}} > 1$).}
%     \label{fig:like_d1}
% \end{figure}



The whole pipeline is applied first in the standard CMB-S4 (classical imager) case with no sub-band splitting ($Nsub=1$) and then for a BI version of the same instrument where each band above 50 GHz is split into a number of sub-bands ranging from 1 to 8 as in Fig~\ref{fig:Polarization_depth}. We account for BI sub-optimality (introduced in section~\ref{sec_instrument_models}) as in~\citep{2020.QUBIC.PAPER2} and Appendix~\ref{appendixA}. We performed an estimation of $r$ for each of our sky realization and we show the result in figure \ref{fig:like_d1} panel {\bf a)}. The increase of $\sigma(r)$ is caused by BI sub-optimality. We see that adding more sub-bands does not add information in this case and, in particular, does not reduce the residual bias on $r$ as it is due to the coarse pixelization on the reconstructed spectral indices that leaves some foreground residuals on the clean CMB maps.


==> III/III-2/III-2-3/decorrelation.tex <==
Let us now consider a more complex dust model that exhibits frequency decorrelation for the dust component ({\bf d6s1}) as in Eq.~\ref{Rl}. This is a more realistic situation than in the previous section and the non-trivial frequency behavior of the dust SED is expected to induce dust residuals in the clean CMB maps when using a component separation parametrization corresponding to {\bf d1s1} that assumes no decorrelation for the dust component (a simple modified black-body).

We have applied the pipeline described above on 500 realizations of model {\bf d6s1}  with $\ell_{\text{corr}} = 10$ (with frequency correlation matrix shown in figure~\ref{fig:Dust_d6_corrl10_correlation_matrix_over_frequency}). As in the previous section, we use our clean CMB maps to reconstruct a value of $r$ for each realization and for each number of sub-bands ($N_{sub}=1$ for a classical imager and $N_{sub}>1$ for a BI). The results are displayed in panel {\bf c)} from figure~\ref{fig:like_d1}. We observe that the range of reconstructed $r$ is dramatically increased by the dust frequency decorrelation, even though we have used a conservative amount of decorrelation with respect to the best current upper-limits from Planck \citep{planck_2020_decorrelation, Planck_2020}. 
For comparison, we show in panel {\bf b)} from figure~\ref{fig:like_d1} the reconstructed vaules of $r$ for the {\bf d1s1} but with an input $r=0.01$.

The {\bf d)}  panel of figure~\ref{fig:like_d1} shows a comparison of the averages and standard deviations of our reconstructed r as a function of the number of sub-bands $N_{sub}$ for the three cases considered here ({\bf d1s1}, $r=0$), ({\bf d1s1}, $r=0.01$), and ({\bf d6s1}, $r=0$). 
For a classical imager (CMB-S4, $N_{sub}=1$), the range of reconstructed $r$, when the input is zero, goes from $7.1\times 10^{-4}\pm 3.2\times 10^{-4}$ ({\bf d1s1}) to $1.3\times 10^{-2}\pm 2\times 10^{-2}$ when unaccounted dust decorrelation is present preventing any detection of primordial B-modes with r below $3\times 10^{-2}$, close to the current upper-limit~\citep{2021PhRvL.127o1301A}.

However, we observe that when using a BI with the same data containing unaccounted foreground decorrelation, the possibility of splitting into several sub-bands at the data analysis level reveals a significant decrease of the average bias and standard deviation of the reconstructed $r$ as one increases the number of reconstructed sub-bands. This reduction of the reconstructed $r$ is not seen with a simpler dust model, be it with $r=0$ or $r=0.01$ where one sees no evolution with the number of reconstructed sub-bands. A similar behavior is shown in figure~\ref{fig:result_r_vs_dust_model} where we vary the dust correlation length. We observe that the reduction of the bias on r due to uncontrolled foreground residuals always decreases when increasing the number of sub-bands. Of course, as expected, the overall amount of bias reduces when increasing the dust correlation length, reaching a similar situation as for {\bf d1s1} for $\ell_{corr} \sim 100$.

The possibility of analysing the same data with a varying number of reconstruction sub-bands, and the observed reduction of the bias when doing so, open the door to using Bolometric Interferometry  for 
controlling foreground residuals contamination in the case of complex dust models, for which a single, deterministic SED is a too crude approximation. However, the behavior observed in figures~\ref{fig:like_d1} and~\ref{fig:result_r_vs_dust_model} is 
found to be significant on the average over a large number of noisy CMB and dust realisations, which is not accessible in the real world. One therefore needs to assess whether the distinct evolution of the reconstructed $r$ with the number of sub-bands a case with no dust residuals (flat evolution) and unaccounted dust residuals (decrease) is significant on a single realization, which the what an experiment has access to.


%  The results of these simulations are shown in the figure~\ref{fig:result_r_vs_dust_model} and shows the results on the recovered best fit value of r for all the simulated instrumental configurations and dust models. Whereas in the d0 and d1 case the results are compatible between all instruments and show no bias, unaccounted dust frequency decorrelation contaminates the CMB signal and can cause a bias on r. However, the increased spectral resolution provided by BI helps reducing the bias and for correlation length $\ell_{corr} > 10$ it even removes it.

% Moreover, when adding spectral imaging, the recovered value of r changes significantly with respect to the single band case (the blue point of BI7 are not compatible with the red ones of S4 for correlation length of the order of 10), thus hinting that the recovered r is not a cosmological signal but the residual due to improper foreground removal.

% Finally, when increasing the correlation length, thus decreasing the deviation from a single-modified black-body, one can see that the results are consistent with the d1 case, as expected in the limit of an infinite $\ell_{corr}$.


% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{figure/d6_recon_r.png}
%     \caption{Likelihoods on $r$ for $N_{\text{sub}}$ = 1, 3, 5 and 8. \comm{Elenia - Why is this likelihood not gaussian (is it obtained from the average Dls)? Are we able to justify it? I suggest to substitute this plot with the one of the average log-like instead, which is fully gaussian}}

%     \comm{Answer - I'm ploting the distribution of each max liklelihood for each reals. I tought that we decided to plot this kind of results.}
%     \label{fig:like_d6_corr15}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[scale=0.30]{figure/rmax_d6_corr15.pdf}
%     \caption{Positions of maximum likelihoods on $r$ (dots) and their $\sigma(r)$ (arrow towards up) for $N_{\text{sub}}$ = 1, 3, 5 and 8.}
%     \label{fig:like_d6_corr15}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figure/Results_on_r_vs_dust_model.pdf}
    \caption{Results on the tensor-to-scalar ratio as a function of the simulated dust model for CMB-S4 and the three BI versions of CMB-S4.  These results indicate that the increased spectral resolution of BI allows one to identify the presence of dust residuals due to frequency decorrelation effects in a way unattenable for a traditional imager. \JCH{redo this plot with histo of the r (Elenia). Also we need to use $\ell$ instead of $l$ + increase the size of the characters. Additionnaly, for now the point do not seem consistent with thos from figure~\ref{fig:like_d1}. SO we need to check this in details.}}
    \label{fig:result_r_vs_dust_model}
\end{figure}


